The VLT-FLAMES survey of massive stars. NGC2004#115: A triple system hosting a possible short period B+BH binary

The star NGC2004#115 in the LMC, originally classified as an (SB1) Be spectroscopic binary, bears some morphological resemblance to the Galactic systems LB-1 and HR 6819, both of which are proposed as either Be+black hole (BH) or Be+stripped He-star systems. Two data-sets (ESO/VLT and SALT) of multi-epoch optical spectra of NGC 2004#115, separated by baseline of $\sim$20 years, lead us conclude it is a triple system hosting an inner binary with a period of 2.92 d, eccentricity $\sim$0.0 and mass function $\sim$0.07 $M_\odot$. The inner binary harbours a B-type star (the primary) with projected rotational velocity of 10km/s, and luminosity $\log L/L_\odot$=3.87, contributing $\sim$60% of the V-band light to the system. The secondary is not detected, while the tertiary, which contributes 40% of the light, is tentatively identified as a less luminous B-type star with high projected rotational velocity. No ellipsoidal light variability is detected, with stringent limits being set by MACHO and Gaia data. Assuming the primary to be a main sequence star yields a mass of 8.6$ M_\odot$, while the additional assumption of synchronous rotation constrains the inclination to be almost pole-on with i~9 degrees, implying the secondary is a BH with a mass of $\sim$25 $M_\odot$. A low mass stripped star with similar luminosity is ruled out as a potential solution as its mass implies a Roche radius that is substantially smaller than the stellar radius. The outer period likely exceeds 120 days and, while the disk-like emission is variable (it is almost absent in the SALT dataset), it may be associated with the inner binary rather than the rapidly rotating tertiary. XMM-Newton provides an upper limit of 5x$10^{33}$ ergs/s on the X-ray flux, consistent with, though not constraining of, the system hosting a quiescent B+BH binary. A number of caveats to this scenario are discussed in the paper.

==> params.tex <==
\begin{table*}
\caption{Derived stellar parameters, absolute abundances and abundances relative to LMC baseline for a range of \% veiling contributions.}
\centering
\begin{tabular}{cccrlrlrlrlrlrlrc}\hline\hline 
\teff & \logg & \vt  & \% & C & $\Delta$(C) & N & $\Delta$(N) & O & $\Delta$(O) & Mg & $\Delta$(Mg) & Si & $\Delta$(Si) \\ \hline
21000 &	3.60 &   0 &	 0\% &   7.22  &  -0.53 &  6.83 &   -0.07 &  8.09 &   -0.26 &  6.63 &   -0.42 &  6.71  &  -0.49 \\
\\
%21000 & 3.75 &   0 &    10\% &   7.30  &  -0.45 &  6.93 &   0.03  &  8.30 &   -0.05 &  6.70 &   -0.35 &  6.92  &  -0.28 \\
21500 & 3.80 &   0 &    10\% &   7.32  &  -0.43 &  6.90 &   0.00  &  8.21 &   -0.14 &  6.74 &   -0.31 &  6.84  &  -0.36 \\
%22000 &	3.85 &	 0 &	10\% &   7.34  &  -0.41 &  6.87 &   -0.03 &  8.12 &   -0.23 &  6.78 &   -0.27 &  6.77  &  -0.43 &  x \\
\\
%21000 &	3.90 &	 0 &	20\% &   7.41  &  -0.34 &  7.08 &   0.18  &  8.51 &   0.16  &  6.78 &   -0.27 &  7.14  &  -0.06 &  1 \\
21500 &	3.95 &	 0 &	20\% &   7.42  &  -0.33 &  7.04 &   0.14  &  8.42 &   0.07  &  6.82 &   -0.23 &  7.07  &  -0.14 \\
%22000 &	4.00 &	 0 &	20\% &   7.42  &  -0.33 &  6.99 &   0.09  &  8.33 &   -0.02 &  6.86 &   -0.19 &  6.99  &  -0.21 &  x \\
%23000 &	4.10 &	 0 &	20\% &   7.46  &  -0.29 &  6.93 &   0.03  &  8.17 &   -0.18 &  6.94 &   -0.11 &  6.85  &  -0.35 &  x \\
\\
%21000 &	4.00 &	 0 &	25\% &   7.47  &  -0.28 &  7.17 &   0.27  &  8.72 &   0.36  &  6.83 &   -0.22 &  7.27  &  0.07  &  x \\
22000 &	4.10 &	 0 &	25\% &   7.48  &  -0.27 &  7.07 &   0.17  &  8.44 &   0.09  &  6.91 &   -0.14 &  7.11  &  -0.09 \\
%23000 &	4.20 &	 0 &	25\% &   7.51  &  -0.24 &  7.00 &   0.09  &  8.28 &   -0.07 &  6.98 &   -0.07 &  6.97  &  -0.23 &  x \\
\\
%21000 &	4.10 &	 0 &	30\% &   7.54  &  -0.21 &  7.27 &   0.37  &  8.77 &   0.42  &  6.87 &   -0.18 &  7.40  &  0.20  &  x \\
%22000 &	4.20 &	 0 &	30\% &   7.54  &  -0.21 &  7.16 &   0.26  &  8.58 &   0.23  &  6.95 &   -0.10 &  7.24  &  0.04  &  x \\
22500 &	4.25 &	 0 &	30\% &   7.55  &  -0.20 &  7.12 &   0.22  &  8.49 &   0.14  &  6.99 &   -0.06 &  7.17  &  -0.03  \\
%23000 &	4.30 &	 0 &	30\% &   7.56  &  -0.19 &  7.07 &   0.17  &  8.41 &   0.06  &  7.03 &   -0.02 &  7.10  &  -0.10 &  1 \\
\hline
\end{tabular}
\label{table:params}
\end{table*}
%PLD: Upper limit: 0%  22kK
%PLD: Upper limit  10% 23kK 
%PLD: Upper limit: 20% 23kK
%PLD: Upper limit: 25% 24kK
%PLD: Upper limit: 30% 25kK

